Tree-like resolution complexity of two planar problems

We consider two CSP problems: the first CSP encodes 2D Sperner's lemma for the standard triangulation of the right triangle on $n^2$ small triangles; the second CSP encodes the fact that it is impossible to match cells of $n \times n$ square to arrows (two horizontal, two vertical and four diagonal) such that arrows in two cells with a common edge differ by at most $45^\circ$, and all arrows on the boundary of the square do not look outside (this fact is a corollary of the Brower's fixed point theorem). We prove that the tree-like resolution complexities of these CSPs are $2^{\Theta(n)}$. For Sperner's lemma our result implies $\Omega(n)$ lower bound on the number of request to colors of vertices that is enough to make in order to find a trichromatic triangle; this lower bound was originally proved by Crescenzi and Silvestri. CSP based on Sperner's lemma is related with the $\rm PPAD$-complete problem. We show that CSP corresponding to arrows is also related with a $\rm PPAD$-complete problem.

==> parts/draft.intro.tex <==
In the paper we consider two problems based on Sperner's lemma and Brouwer's theorem.

In the first problem we have a triangle, which is divided on small ones. Each vertex of small triangles is colored by one of three colors. We know that vertices of the large triangle are colored by three different colors; each vertex, which lies on a side of the large triangle, is colored by a color of either one or another end of the side. Sperner's lemma states that there exists a small triangle, all vertices of whom is colored by three different colors. We call such a triangle as \textit{trichromatic}.

We investigate the next problem: given an access to a vertex coloring find a trichromatic triangle.
Our first point of interest is the decision-tree complexity of the problem.
For the fixed triangulation we present each strategy for looking a trichromatic triangles by tree.
An inner node of the tree contains a vertex, which color should be asked. Each outgoing edge is labeled
by possible answer. So, for example, if one recieves answer Red, she should go by corresponding edge and ask
the next vertex. Each leaf of the tree contains a correct answer.

We show that lower bound $2^{\Omega(n)}$ on the tree size, where $n$ is the measure of the triangulation.

The next problem is inspired by Brower's theorem. We consider a $n \times n$ square and fill each cell by an arrow
from set $\{\al, \alu, \au, \aru, \ar, \ard, \ad, \ald\}$. The only restriction is all arrows on the boundary of the square
should be directed inside. It follows from Brower's theorem, that there are two cells adjucent by edge, which contain arrows
with the angle between them more than $45^\circ$.

Given an access to an assignment of arrows to cells one should find such two cells. 
We prove that decision-tree complexity here is $2^\Theta(n)$.

The second point of interest is $\PPAD$-completeness of these problem.
We present a coloring or cell assignment by a polynomial Turing machine. The machine receives coordinates of an element and
returns assigned value (color or arrow). It is known for such setting that Sperner's lemma is $\PPAD$-complete. We prove
that problem on arrows is $\PPAD$-complete too.
